Learning One Class Representations for Face Presentation Attack Detection using Multi-channel Convolutional Neural Networks

Face recognition has evolved as a widely used biometric modality. However, its vulnerability against presentation attacks poses a significant security threat. Though presentation attack detection (PAD) methods try to address this issue, they often fail in generalizing to unseen attacks. In this work, we propose a new framework for PAD using a one-class classifier, where the representation used is learned with a Multi-Channel Convolutional Neural Network (MCCNN). A novel loss function is introduced, which forces the network to learn a compact embedding for bonafide class while being far from the representation of attacks. A one-class Gaussian Mixture Model is used on top of these embeddings for the PAD task. The proposed framework introduces a novel approach to learn a robust PAD system from bonafide and available (known) attack classes. This is particularly important as collecting bonafide data and simpler attacks are much easier than collecting a wide variety of expensive attacks. The proposed system is evaluated on the publicly available WMCA multi-channel face PAD database, which contains a wide variety of 2D and 3D attacks. Further, we have performed experiments with MLFP and SiW-M datasets using RGB channels only. Superior performance in unseen attack protocols shows the effectiveness of the proposed approach. Software, data, and protocols to reproduce the results are made available publicly.

==> Makefile <==
# Created by Andre Anjos <andre.anjos@idiap.ch>
# Tue 18 Apr 2017 11:50:17 CEST

# Builds the LaTeX project as a PDF document

TEXFILE=mcocm_tifs.tex
PDFFILE=$(TEXFILE:%.tex=%.pdf)

%.pdf: %.tex
	pdflatex $(@:%.pdf=%.tex); \
	bibtex $(@:%.pdf=%); \
	pdflatex $(@:%.pdf=%.tex); \
	pdflatex $(@:%.pdf=%.tex);

all: $(PDFFILE)

.PHONY: clean

clean:
	@rm -vf $(shell find . -name "*~")
	@rm -vf *.log *.lot *.lof *.loa *.toc *.idx *.inc *.ilg *.ind *.blg
	@rm -vf *.aux *.glo *.dvi *.ps main.pdf *.out *.brf $(PDFFILE)

